Predictive Collective Variable Discovery with Deep Bayesian Models

Extending spatio-temporal scale limitations of models for complex atomistic systems considered in biochemistry and materials science necessitates the development of enhanced sampling methods. The potential acceleration in exploring the configurational space by enhanced sampling methods depends on the choice of collective variables (CVs). In this work, we formulate the discovery of CVs as a Bayesian inference problem and consider the CVs as hidden generators of the full-atomistic trajectory. The ability to generate samples of the fine-scale atomistic configurations using limited training data allows us to compute estimates of observables as well as our probabilistic confidence on them. The methodology is based on emerging methodological advances in machine learning and variational inference. The discovered CVs are related to physicochemical properties which are essential for understanding mechanisms especially in unexplored complex systems. We provide a quantitative assessment of the CVs in terms of their predictive ability for alanine dipeptide (ALA-2) and ALA-15 peptide.

==> figures/aevb_scheme_2.tex <==

\newlength\spNet
\spNet=1.cm
\newlength\nodedist
\nodedist=.6cm

\newcommand{\scaletikz}{0.6}

\begin{tikzpicture}[scale=0.7, node distance = .8cm, auto,
    block/.style={
      rectangle,
      draw,%=blue,
      thick,
      fill=orange!10,
      text width=.5cm,
      text centered,
      align=center,
      rounded corners,
      minimum height=6em
    },
    line/.style={black, draw, opacity=0.5}
]

    %%%%%%%%%%%%%%%%%%%%
    %% ENCODER
    %%%%%%%%%%%%%%%%%%%%
    
    % encoder network
    \node [block] (l_1) {$l_{\boldsymbol \phi}^{(1)}$};
    \node [block, right of=l_1] (a_1) {$a^{(1)}$};
    \node [block, right of=a_1, node distance = \spNet] (l_2) {$l_{\boldsymbol \phi}^{(2)}$};
    \node [block, right of=l_2] (a_2) {$a^{(2)}$};
    \node [block, right of=a_2, node distance = \spNet] (l_3) {$l_{\boldsymbol \phi}^{(3)}$};
    %\node [block, right of=l_3] (a_3) {$a_{\boldsymbol \phi}^{(3)}$};
    %\node [block, right of=a_2, node distance = \spNet] (l_3) {$l_{\boldsymbol \phi}^{(1)}$};
    \node [block, right of=l_3] (a_3) {$a^{(3)}$};
    
    % encoder input
    \node [text width=0.5cm, left of=l_1, node distance = 1cm] (input) {$\boldsymbol x^{(i)}$};
    
    % encoder mu
    \node [block, above right=-0.5cm and \nodedist of a_3] (l_4) {$l_{\boldsymbol \phi}^{(4)}$};
    \node [text width=0.5cm, right of=l_4, node distance = 1cm] (mu) {$\boldsymbol \mu\inphi(\boldsymbol x^{(i)})$};
    
    % encoder logvar
    \node [block, below right=-0.5cm and \nodedist of a_3] (l_5) {$l_{\boldsymbol \phi}^{(5)}$};
    \node [text width=0.5cm, right of=l_5, node distance = 1cm] (logvar) {$\log \boldsymbol \sigma\inphi^2(\boldsymbol x^{(i)})$};
    
    % https://tex.stackexchange.com/questions/71478/how-to-center-one-node-exactly-between-two-others-with-tikz
    \path (mu) -- (logvar) node[midway] (post) {$q_{\boldsymbol \phi}(\boldsymbol z^{(i)} | \bxi ) = \mathcal N\left(\boldsymbol z^{(i)}| \boldsymbol \mu\inphi(\bxi),\boldsymbol{S}_{\boldsymbol{\phi}}(\bxi)\right)$};
    %\node (normal) at ($(mu)!0.5!(logvar)$) {$q_{\boldsymbol \phi}(\boldsymbol z^{(i)} ) = \mathcal N(\boldsymbol z^{(i)}| \boldsymbol \mu^{(i)}, \boldsymbol \sigma^{2 (i)} \boldsymbol I)$};
    
    % from https://tex.stackexchange.com/questions/199065/tikz-connecting-nodes-with-multiple-lines
    \foreach \x in {.0,1.} {
    \draw[dashed]($(a_1.north east)!\x!(a_1.south east)$) -- ($(l_2.north west)!\x!(l_2.south west)$);
    \draw[dashed]($(a_2.north east)!\x!(a_2.south east)$) -- ($(l_3.north west)!\x!(l_3.south west)$);
    \draw[dashed]($(a_3.north east)!\x!(a_3.south east)$) -- ($(l_4.north west)!\x!(l_4.south west)$);
    \draw[dashed]($(a_3.north east)!\x!(a_3.south east)$) -- ($(l_5.north west)!\x!(l_5.south west)$);
    }
    
    % mu and logvar to posterior distribution
    \draw[dashed, ->](mu) -> (post);
    \draw[dashed, ->](logvar) -> (post);
    
    
    %%%%%%%%%%%
    % DECODER
    %%%%%%%%%%%
    
    % decoder network
    \node [block, below right=3cm and 5.cm of l_5, ] (decl_1) {$l^{(1)}_{\boldsymbol \theta}$};
    \node [block, left of=decl_1] (deca_1) {$\tilde{a}^{(1)}$};
    
    \node [block, left of=deca_1, node distance = \spNet] (decl_2) {$l^{(2)}_{\boldsymbol \theta}$};
    \node [block, left of=decl_2] (deca_2) {$\tilde{a}^{(2)}$};
    
    \node [block, left of=deca_2, node distance = \spNet] (decl_3) {$l^{(3)}_{\boldsymbol \theta}$};
    \node [block, left of=decl_3] (deca_3) {$\tilde{a}^{(3)}$};
    
    % decoder mu
    \node [block, left of=deca_3, node distance = \spNet] (decl_4) {$l^{(4)}_{\boldsymbol \theta}$};
    \node [text width=0.9cm, left of=decl_4, node distance = 1.3cm] (decmu) {$\boldsymbol \mu_{\boldsymbol \theta}(\boldsymbol z)$};
    % decoder logvar
    %\node [block, below left=-0.5cm and \nodedist of deca_3] (decl_5) {$l^5_{\boldsymbol \theta}$};
    %\node [text width=0.5cm, left of=decl_5, node distance = 1cm] (declogvar) {$\log \boldsymbol \sigma^2(\boldsymbol z)$};
    
    % decoder input
    \node [text width=2.cm, right of=decl_1, node distance = 1.5cm] (decinput) {$\boldsymbol z \sim p_{\boldsymbol \theta}(\boldsymbol z)$};
    
    % https://tex.stackexchange.com/questions/71478/how-to-center-one-node-exactly-between-two-others-with-tikz
    %\path (decmu) -- (declogvar) 
    \node[left of=decmu, node distance = 3.3cm] (pred) {$p_{\boldsymbol \theta}(\boldsymbol x | \boldsymbol z ) = \mathcal N\left(\boldsymbol x | \boldsymbol \mu_{\boldsymbol \theta}(\bz), \boldsymbol{S}_{\boldsymbol{\theta}} \right)$};
    %\node (normal) at ($(mu)!0.5!(logvar)$) {$q_{\boldsymbol \phi}(\boldsymbol z^{(i)} ) = \mathcal N(\boldsymbol z^{(i)}| \boldsymbol \mu^{(i)}, \boldsymbol \sigma^{2 (i)} \boldsymbol I)$};
    
    \foreach \x in {.0,1.} {
    \draw[dashed]($(deca_1.north west)!\x!(deca_1.south west)$) -- ($(decl_2.north east)!\x!(decl_2.south east)$);
    \draw[dashed]($(deca_2.north west)!\x!(deca_2.south west)$) -- ($(decl_3.north east)!\x!(decl_3.south east)$);
    \draw[dashed]($(deca_3.north west)!\x!(deca_3.south west)$) -- ($(decl_4.north east)!\x!(decl_4.south east)$);
    %\draw[dashed]($(deca_3.north west)!\x!(deca_3.south west)$) -- ($(decl_5.north east)!\x!(decl_5.south east)$);
    }
    
    % mu and logvar to posterior distribution
    \draw[dashed, ->](decmu) -> (pred);
    \draw[dashed, ->](decl_4) -> (decmu);
    
    %\draw[dashed, ->](declogvar) -> (pred);
     
    \path [line, red, dashed, <->, very thick] ([xshift=0.8cm]post.south west) to [out=330,in=90] %node[above,xshift=1cm,yshift=-0.9cm] {$-\sum_{i=1}^N D_{KL}(q\inphi(\bzi|%\bxi) || p\inth(\bz)) $} 
    (decinput);
    
    \path [line, blue, dashed, <->, very thick] (input) to [out=270,in=145] node[above,xshift=7.cm,yshift=-1.2cm, opacity=1., black] {$\mathcal L(\btheta, \bphi; \bX) =  
    \sum_{i=1}^N
    {\color{blue}    
    \mathbb E_{q\inphi(\bzi|\bxi)} [\log p\inth(\bxi|\bzi) ]
    }
    -\sum_{i=1}^N
    {\color{red}    
    D_{KL}\left( q\inphi(\bzi|\bxi) || p\inth(\bz) \right)
    }
    $
    }  ([xshift=.5cm]pred.north west);

    \draw [black,thick, dotted, opacity=0.5]  ($(l_1.north west)+(-1.5,3.)$)  rectangle ($( post.east)+(0.5,-4.5)$);
    
    \node (encoder) at ($(l_1.north west)+(-0.5, 2.5)$) [minimum width=2cm,minimum height=0.1cm,label={ Encoder},anchor=south] {};
    
    
    
    \draw [black,thick,dotted, opacity=0.5]  ($(pred.north west)+(-0.7, 1.5)$)  rectangle ($( decinput.east)+(0.5,-2)$);
    
    \node (decoder) at ($(pred.north west)+(+0.2, 1.0)$) [minimum width=2cm,minimum height=0.1cm,label={ Decoder},anchor=south] {};
    
    

\end{tikzpicture}




==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}



% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}
